Online Robustness Training for Deep Reinforcement Learning

In deep reinforcement learning (RL), adversarial attacks can trick an agent into unwanted states and disrupt training. We propose a system called Robust Student-DQN (RS-DQN), which permits online robustness training alongside Q networks, while preserving competitive performance. We show that RS-DQN can be combined with (i) state-of-the-art adversarial training and (ii) provably robust training to obtain an agent that is resilient to strong attacks during training and evaluation.

==> figures/defenses.tex <==
\begin{figure}[ht]
\begin{center}
    \includegraphics[height=1cm]{figures/defenses_.pdf}
  \end{center}
  \caption{Different instantiation for \defend in \cref{fig:alg}. \cref{sec:studnet} discusses Student-DQN without any defense and \cref{sec:defenses} turns Student-DQN into \system by applying either adversarial training or provably robust training.} \label{fig:defenses}
\end{figure}

%
%
%
%


==> related.tex <==
%
%

\paragraph{Adversarial Robustness of Deep Q Learning}
\cite{robustDeep} uses adversarial examples to train a deep Q learning agent and improve its experimental robustness. Their evaluation is limited to agents with few input parameters such as speed and velocity. \cite{whatDoesntKillyou} noticed that adversarial training can prevent learning -- especially in games with a high number of input variables such as the frames in Atari games.
\cite{behzadan2017vulnerability} further demonstrated this effect could be intentionally amplified to prevent learning by an adversary.


\paragraph{Robustness of Deep RL in different contexts}
Deep RL is closely linked to control theory, where robustness against a wide class of small perturbations to the input is studied. \cite{robustAdversarialRL, mandlekar2017adversarially, gu2018adversary, robustAuto} all train on perturbed data points or in the presence of an adversary in order to increase model robustness or generalization. These works focus on actor critic methods rather than Q-learning. \cite{onlinerobustness} use a similar approach, where they extend hierarchical reinforcement learning, such that the agent is robust against perturbations during learning. They motivate their approach by providing theoretical guarantees.

\cite{shashua2017deep} train a DQN that avoids the worst-case outcome and performs well in the presence of non-deterministic environments by using an extended Kalman-Filter. However, their Kalman-update requires multiplication of matrices of size quadratic in the total number of weights and thus does not scale.
%

\paragraph{Distillation}
\cite{defensiveDistillation} first proposed that distilling a neural network by training the same architecture with the probability vector outputs of the original network might act as a defense against adversarial examples.
%

\cite{linCollaborativeDeepReinforcement2017} uses distillation to improve reinforcement learning itself by introducing the collaborative asynchronous advantage actor-critic algorithm (cA3C). Their method allows for knowledge transfer between agents in cases where multiple agents are playing simultaneously in different environments with potentially different tasks.

Similar to distillation, \cite{chenAgentAwareDropoutDQN2017} use a pre-defined rule-based teacher policy to assist a deep RL system.  They introduce a new DQN algorithm which predicts when to consult the teacher and how to learn from it.

\paragraph{Provably robust training}
\cite{raghunathan2018certified} introduced a technique to train networks to be certifiably robust (though again limited to small networks).
Multiple recent techniques have been developed since to train increasingly larger networks to be certifiably robust including \cite{kolter2018provable, diffai, dvijotham2018training, wong2018scaling}.
These techniques represent different points in the spectrum of accuracy, training speed certifiable robustness and experimental robustness.

